FluidLab: A Differentiable Environment for Benchmarking Complex Fluid Manipulation

Humans manipulate various kinds of fluids in their everyday life: creating latte art, scooping floating objects from water, rolling an ice cream cone, etc. Using robots to augment or replace human labors in these daily settings remain as a challenging task due to the multifaceted complexities of fluids. Previous research in robotic fluid manipulation mostly consider fluids governed by an ideal, Newtonian model in simple task settings (e.g., pouring). However, the vast majority of real-world fluid systems manifest their complexities in terms of the fluid's complex material behaviors and multi-component interactions, both of which were well beyond the scope of the current literature. To evaluate robot learning algorithms on understanding and interacting with such complex fluid systems, a comprehensive virtual platform with versatile simulation capabilities and well-established tasks is needed. In this work, we introduce FluidLab, a simulation environment with a diverse set of manipulation tasks involving complex fluid dynamics. These tasks address interactions between solid and fluid as well as among multiple fluids. At the heart of our platform is a fully differentiable physics simulator, FluidEngine, providing GPU-accelerated simulations and gradient calculations for various material types and their couplings. We identify several challenges for fluid manipulation learning by evaluating a set of reinforcement learning and trajectory optimization methods on our platform. To address these challenges, we propose several domain-specific optimization schemes coupled with differentiable physics, which are empirically shown to be effective in tackling optimization problems featured by fluid system's non-convex and non-smooth properties. Furthermore, we demonstrate reasonable sim-to-real transfer by deploying optimized trajectories in real-world settings.

==> 1_abstract.tex <==

\begin{abstract}


Humans need to perform various manipulation tasks in their daily life where they need to interact with fluids: doing latte art, making ice creams, scooping a floating object out of water, etc. Previous research in robotic manipulation involving fluids mostly consider relatively simple settings and with a single fluid phase, such as water pouring or scooping. More realistic manipulation tasks with complex configurations of fluid bodies and their interactions have been rarely studied in a comprehensive way, and are extremely challenging due to their high-dimensional observation space and the highly nonlinear underlying fluid dynamics. In this work, we study the problem of \textit{complex fluid manipulation} with more realistic task settings and complex goal configurations. We introduce \textit{FluidLab}, a simulation environment with a diverse set of manipulation tasks involving complex fluid dynamics. These tasks concern not only different phases of fluids, but also their interactions with other non-fluid bodies. Since modeling such a variety of material types and coupling between them are not supported by existing simulation engines, we developed \textit{FluidEngine}, the underlying physics engine of FluidLab that supports simulating a wide range of materials and coupling between them. FluidEngine is implemented in a fully \textit{differentiable} manner, providing useful gradient information for downstream optimization tasks. We evaluate both RL-based algorithms and optimization-based methods in FluidLab, and highlight several challenges for existing methods for manipulating fluids. In addition, we propose several optimization techniques specific to the domain of fluid manipulation, which when combined with differentiable physics, could be effective in solving some challenging tasks with unconvex and non-smooth optimization landscapes. FluidLab and FluidEngine will be publicly available\footnote{Project page: \href{https://sites.google.com/view/fluidlab}{\texttt{https://sites.google.com/view/fluidlab}}}.
\end{abstract}


==> 1_abstract_2.tex <==
%% Bo's version
\begin{abstract}
%
Human manipulates various kinds of fluid in their daily life. Most of these manipulations are for cooking, dining, and food processing, including creating latte art, scooping a tofu piece from soap, rolling an ice cream cone, to name just a few. Using AI and robots to augment or replace human labors in these housework settings remain as a challenging task due to the fluid's multifaceted complexities. Existing learning frameworks were mainly focused on manipulating fluid governed by an ideal, Newtonian model in simple tasks (e.g., pouring water into a container). However, the vast majority of real-world fluid systems manifest their scene complexities in terms of the fluid's nonlinear properties (e.g., non-Newtonian viscosity) and the solid's intricate geometries (e.g., a thin, curved scoop), both of which were well beyond the scope of the current literature. \gc{In order to evaluate robot learning models on understanding and interacting with complex fluid systems, a comprehensive virtual platform with well-established tasks, environments, and evaluation metrics is needed. }
%
We propose to investigate these \textit{complex fluid manipulation} problems by establishing a novel platform, \textit{FluidLab}, facilitated jointly by our versatile and interactive fluid simulation backend and domain-specific optimization frontend. %Our goal is to address the gap between the current fluid simulation tools and the diverse real-world manipulation tasks. 
At the heart of our platform is a fully differentiable fluid simulator, \textit{FluidEngine}, to support parallel simulations and gradient calculations for a wide range of complex fluid models and solid-fluid interactions. 
%
On the optimization end, we implemented RL-based algorithms and gradient-based optimization methods by highlighting several challenges in learning fluid manipulations with existing methods. We also proposed several domain-specific optimization schemes to tackle fluid optimization problems featured by highly non-convex and non-smooth properties. 
%
Based on these simulation and optimization modules, we proposed ten novel benchmarking tasks for complex fluid manipulation, such as XXX, XXX, and XXX, which were all infeasible to testify with the previous simulation and learning toolsets. 
\end{abstract}


==> 1_abstract_3.tex <==

\begin{abstract}


Humans manipulate various kinds of fluid in their everyday life: creating latte art, scooping floating objects from water, rolling an ice cream cone, etc. Using robots to augment or replace human labors in these daily tasks remain as a challenging task due to the multifaceted complexities of fluids. Previous research in robotic fluid manipulation mostly consider fluids governed by an ideal, Newtonian model in simple task settings (e.g., pouring water into a container). 
However, the vast majority of real-world fluid systems manifest their complexities in terms of the fluid's complex material behaviors (e.g., elastoplastic deformation) and multi-component interactions (e.g. coffee and frothed milk when making latte art), both of which were well beyond the scope of the current literature. 
To evaluate robot learning algorithms on understanding and interacting with such
complex fluid systems, a comprehensive virtual platform with versatile simulation
capabilities and well-established tasks is needed. In this work, we introduce \textit{FluidLab}, a simulation environment with a diverse set of manipulation tasks involving complex fluid dynamics. These tasks address interactions between solid and fluid as well as among multiple fluids. At the heart of our platform is a fully differentiable physics simulator, \textit{FluidEngine}, providing GPU-accelerated simulations and gradient calculations for various material types and their couplings, extending the scope of the existing differentiable simulation engines. 
We identify several challenges for fluid manipulation learning by evaluating a set of reinforcement learning and trajectory optimization methods on our platform.
%We evaluate both RL-based algorithms and trajectory-optimization methods in FluidLab, and highlight several challenges in learning fluid manipulations with existing methods. 
To address these challenges, we propose several domain-specific optimization schemes coupled with differentiable physics, with our particular focus on tackling optimization problems featured by fluid systems' non-convex and non-smooth properties. FluidLab and FluidEngine will be publicly available. Demos can be viewed on our project page \footnote{Project Page: \url{https://sites.google.com/view/fluidlab}}.
\end{abstract}


==> 1_abstract_final.tex <==

\begin{abstract}


Humans manipulate various kinds of fluids in their everyday life: creating latte art, scooping floating objects from water, rolling an ice cream cone, etc. Using robots to augment or replace human labors in these daily settings remain as a challenging task due to the multifaceted complexities of fluids. Previous research in robotic fluid manipulation mostly consider fluids governed by an ideal, Newtonian model in simple task settings (e.g., pouring water into a container). 
However, the vast majority of real-world fluid systems manifest their complexities in terms of the fluid's complex material behaviors (e.g., elastoplastic deformation) and multi-component interactions (e.g. between coffee and frothed milk when making latte art), both of which were well beyond the scope of the current literature. 
To evaluate robot learning algorithms on understanding and interacting with such
complex fluid systems, a comprehensive virtual platform with versatile simulation
capabilities and well-established tasks is needed. In this work, we introduce \textit{FluidLab}, a simulation environment with a diverse set of manipulation tasks involving complex fluid dynamics. These tasks address interactions between different fluid bodies, as well as their interactions with other non-fluid materials. At the heart of our platform is a fully differentiable physics simulator, \textit{FluidEngine}, providing GPU-accelerated simulations and gradient calculations for various material types and their couplings, which are not supported by existing simulation engines. 
We identify several challenges for fluid manipulation learning by evaluating a set of reinforcement learning and trajectory optimization methods on our platform.
In addition, we propose several domain-specific optimization schemes coupled with differentiable physics, which are empirically shown to be effective in  tackling the proposed challenging tasks featured by fluid system's non-convex and non-smooth properties. FluidLab and FluidEngine will be publicly available. Demos can be viewed on our project page \footnote{Project page: \href{https://sites.google.com/view/fluidlab}{\texttt{https://sites.google.com/view/fluidlab}}}.


\end{abstract}


==> 2_intro.tex <==
\section{Introduction} 
Imagine you are fishing in a peaceful lake. Your hat falls into the water, and starts to float out of reach. In order to get it back, you use your hands to paddle the water gently, making a current that pulls the the hat back into reach. Under this scenario, the water functions as a transmitting medium to accomplish the manipulation task. In fact, from making latte art and washing dishes, to designing smoke ventilation systems and pouring ketchup to chips, many of our everyday tasks involve interacting with different types of fluids, as shown in Figure \ref{fig:life}. However, performing these tasks are still beyond reach of today's robotic systems due to several major challenges. First, it requires a high dimensional state space to fully describe a system with fluids in an informative way \citep{lin2020softgym}. Second, such systems have highly unstructured and complex underlying dynamics \citep{schenck2018spnets}. Third, a wide spectrum of different fluid types with a great variation in their properties \todo{Bo: some citations?} are present in our life. For example, while ketchup and smoke both share the first two aforementioned challenges, they also behave in a drastically different way.

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{figures/life.png}
\caption{We encounter various manipulation tasks involving fluids in everyday life. Some examples are shown here. From left to right: making latte art, stirring coffee, making ice creams, designing smoke ventilation systems.}
\label{fig:life}
\end{figure*}

Past decades have witnessed rapid progresses in robotic control and manipulation. Robotic systems today are able to perform reasonably well in a wide range of manipulation tasks including object pushing \citep{yu2016more, li2018push, tung20203d}, grasping and pick-and-place \citep{kleeberger2020survey, zeng2020transporter, shridhar2022cliport}, dexterous and in-hand manipulation \citep{andrychowicz2020learning, chen2022system}, and even furniture assembly \citep{suarez2018can, lee2021ikea}. However, most of these tasks mainly consider rigid objects and focus on goal configurations represented as inter-object spatial relationships. In recent years, there has been a developing interest in manipulating deformable and articulated objects \citep{nair2017combining, schenck2018spnets, li2018learning, lin2020softgym, huang2021plasticinelab, lin2022diffskill, wu2021vat}, where intra-body configurations and appearances of these objects are taken into account during manipulation. Some work among them also cover manipulation tasks involving fluids \citep{ma2018fluid, lin2020softgym, antonova2022rethinking}, but mostly adopts relatively simple task settings, and usually considers tasks with a single-phase fluid, such as pouring water \citep{schenck2018spnets, lin2020softgym, sermanet2018time} or scooping objects from water \citep{Daniel2022toolflow, antonova2022rethinking}. In this work, we aim to take one step further and study the problem of \textit{complex fluid manipulation} with more challenging task settings and complex goal configurations.

To this end, we propose \textit{FluidLab}, a simulation environment with a comprehensive set of manipulation tasks involving various types of fluids. These tasks are motivated by scenarios encountered in our daily life, and consider both interactions within a multi-phase fluid body, as well as coupling between fluid and non-fluid bodies. Building such an environment poses a major challenge to the simulation capability: fluids encountered in our life consist of a wide spectrum of materials with different properties; in addition, simulating these tasks also requires modeling interactions with other non-fluid bodies. For example, coffee is \textit{non-viscous Newtonian} liquid, frothed milk behaves as \textit{viscous Newtonian} liquid (Figure \ref{fig:life}, A), while ice-cream is a type of \textit{non-Newtonian} fluid (Figure \ref{fig:life}, C); when stirring a cup of coffee, we use a \textit{rigid} spoon to manipulate the coffee (Figure \ref{fig:life}, B). However, there lacks a simulation engine in the research community that supports such a wide variety of materials and coupling between them. Therefore, we developed our own physics engine, named \textit{FluidEngine}, to simulate the tasks proposed in FluidLab. FluidEngine is a general-purpose physics simulator that supports modeling solid, liquid and gas, covering materials including elastic, plastic and rigid objects, Newtonian and non-Newtonian liquid, as well as smoke or air. FluidEngine is developed using Taichi \citep{hu2019taichi}, a domain-specific language embedded in Python, and supports massive parallelism on GPUs. In addition, it is implemented in a fully \textit{differentiable} manner, providing useful gradient information for downstream optimization tasks. Notably, closest to FluidEngine is Nvidia FleX \citep{macklin2014unified}, a physics engine that supports both rigid and deformable objects and is widely used in a variety of manipulation environments \citep{lin2020softgym, gan2020threedworld, schenck2018spnets}. However, FleX doesn't support simulating plastic materials and air, and is not differentiable. FluidEngine follows the standard OpenAI Gym API \citep{brockman2016openai} and also comes with a user-friendly Python interface for building custom environments. In addition, we provide a GPU-accelerated renderer developed with OpenGL, providing realistic image rendering in real-time and opening possibilities for sim-to-real transfer in the future. We discuss the details of FluidEngine in Section \ref{sec:fluidengine} and the tasks proposed in FluidLab in Section \ref{sec:fluidlab}. 

We evaluate several state-of-the-art Reinforcement Learning algorithms and optimization methods in FluidLab, and show the \todo{blah blah}. In addition, since differentiable physics has proved useful in many rigid-body and soft-body robotic tasks \citep{xu2021end, lin2022diffskill, xu2022accelerated, li2022contact}, it is desirable to extend it to fluid manipulation tasks. However, supporting such a wide spectrum of materials present in FluidLab in a differentiable way is extremely challenging, and optimization using the gradients is also difficult due to the highly non-smooth optimization landscapes of the proposed tasks.  We propose various techniques that are generally applicable to the context of fluids, making our simulation fully differentiable and providing useful methods to utilize these gradients for downstream optimizations tasks, even with highly unconvex landscapes. We demonstrate that our proposed techniques, combined with differentiable physics, could be effective in solving a set of challenging tasks, even in those with highly unstable fluids, such as air. 


In summary, the contributions of this work are as follows:

\begin{itemize}
  % \item We formally formulate the problem of \textit{fluid manipulation}, categorize a set of complex robotic manipulation problems involving fluids under this formulation, and systematically study them.
  \item We propose \textit{FluidLab}, a set of standardized manipulation tasks for systematically study the problem of \textit{complex fluid manipulation} with challenging task settings and complex goal configurations.
 
  \item We present \textit{FluidEngine}, the underlying physics engine of FluidLab that makes it possible to model various material types required in FluidLab's tasks. To the best of our knowledge, it is the first-of-its-kind physics engine that supports such a wide spectrum of materials and allows multi-way coupling \todo{bo: is this phrase correct?} between them, while being \textit{fully differentiable}.
  
   \item We benchmark existing RL algorithms and optimization approaches, and propose techniques that make differentiable physics useful in solving a set of challenging tasks. Our experiments highlight several challenges for existing methods. We hope FluidLab could inspire future research to develop better methods for solving complex fluid manipulation tasks.
\end{itemize}



==> 2_intro_2.tex <==
\section{Introduction} 
%Bo: I am not sure if we need this example... Kind of complicated
%Imagine you are fishing in a peaceful lake. Your hat falls into the water, and starts to float out of reach. In order to get it back, you use your hands to paddle the water gently, making a current that pulls the the hat back into reach. Under this scenario, the water functions as a transmitting medium to accomplish the manipulation task. In fact, 
\gc{My biggest concerns: our main contribution is a virtual environment for complex fluid manipulation. We do not address the challenging real world robot fluid manipulation now.  So we should first explain why we need a virtual environment for that, why it is difficult to create and how it will eventually benefit real world applications.}

From making latte art in a coffee mug to squeezing ketchup onto potato chips, humans interact with different types of fluids everyday (see examples in Figure \ref{fig:life}). However, performing these tasks are still beyond the reach of today's housework robots due to three major challenges.
\todo{Bo: These three challenges need some careful pass. I could not distinguish the first two challenges. Each challenge requires some brief explaination.}
\todo{Bo: my two cents on structuring these challenges: (1) fluid is complicated (e.g., material, many DoFs, evolving shape and topology, etc., focusing on simulating fluid itself); (2) environment is unknown (simulating fluid and object interactions); (3) high dimensional space for solution search in optimization.}
%
First, it requires a high dimensional state space to fully describe a system with fluids in an informative way \citep{lin2020softgym}. 
%
Second, such systems have highly unstructured and complex underlying dynamics \citep{schenck2018spnets}. 
%
Third, fluid systems exhibit a wide spectrum of material properties and phase models, ranging from air \cite{TODO} to liquid \cite{TODO} to granular and multi-phase flow \cite{TODO}. 
%
For example, although both water and smoke are categorized as incompressible fluid because of the same Navier--Stokes Equations to be solved, manipulating these two mediums in different physical contexts require drastically different models and strategies. 

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{figures/life.png}
\caption{We encounter various manipulation tasks involving fluids in everyday life. Left column: real-world scenarios including making latte art, making ice creams and designing air ventilation systems. Right column: simulation tasks in FluidLab involving latte art, ice-creams and indoor air circulation.}
\label{fig:life}
\end{figure*}

\todo{Bo: This paragraph was very nicely written. My only concern is it sounds like a related-work paragraph, which is a little bit off from the main story line. I guess it is okay for now. One possible strategy is to combine the first two paragraphs.}
Past decades have witnessed rapid progresses in robotic control and manipulation. Robotic systems today are able to perform reasonably well in a wide range of manipulation tasks including object pushing \citep{yu2016more, li2018push, tung20203d}, grasping and pick-and-place \citep{kleeberger2020survey, zeng2020transporter, shridhar2022cliport}, dexterous and in-hand manipulation \citep{andrychowicz2020learning, chen2022system}, and even furniture assembly \citep{suarez2018can, lee2021ikea}. However, most of these tasks mainly consider rigid objects and focus on goal configurations represented as inter-object spatial relationships. In recent years, there has been a developing interest in manipulating deformable and articulated objects \citep{nair2017combining, schenck2018spnets, li2018learning, lin2020softgym, huang2021plasticinelab, lin2022diffskill, wu2021vat}, where intra-body configurations and appearances of these objects are taken into account during manipulation. Some works among them also cover manipulation tasks involving fluids \citep{ma2018fluid, lin2020softgym, antonova2022rethinking}, but mostly adopts relatively simple task settings, and usually considers tasks with a single-phase fluid, such as pouring water \citep{schenck2018spnets, lin2020softgym, sermanet2018time} or scooping objects from water \citep{Daniel2022toolflow, antonova2022rethinking}. In this work, we aim to take one step further and study the problem of \textit{complex fluid manipulation} with more challenging task settings and complex goal configurations. \gc{previous work already work on real robot, why can we say our virtual environment take one step further?}

We propose \textit{FluidLab} as a new simulation platform to enable robots to learn complex fluid manipulation skills toward real-world applications. On this platform, we provide a new set of manipulation tasks that were impractical in the previous literature. These tasks are motivated by scenarios encountered in our daily life, and consider both interactions within a multi-phase fluid body \todo{Bo: What does "multi-phase" mean here? liquid and air?}, as well as coupling between fluid and solids. Building such an environment poses a major challenge to the simulation capability: fluids encountered in our life consist of a wide spectrum of materials with different properties; in addition, simulating these tasks also requires modeling interactions with other non-fluid bodies. 
% an example
For example, coffee is a kind of (mostly inviscid) \textit{Newtonian} liquid; frothed milk behaves as \textit{viscous Newtonian} liquid (i.e., with a constant viscosity that does not change with stress) (Figure \ref{fig:life}, A), while ice cream is a type of \textit{non-Newtonian} fluid (in particular, a shear-thinning fluid with its viscosity decreasing as the local stress increasing) (Figure \ref{fig:life}, C); when stirring a cup of coffee, we use a \textit{rigid} spoon to manipulate the coffee (Figure \ref{fig:life}, B). \todo{Bo: Why A, C, and B, not A, B, C?}
%
However, there lacks a simulation engine in the research community that supports such a wide variety of materials and coupling between them. 
%
\todo{Bo: from here to the end we talk about fluid engine. It is a bit too long. I believe many sentences can go to related work.}
Therefore, we developed our own physics engine, named \textit{FluidEngine}, \bo{Bo: FluidEngine does not sound like an attractive name...} to simulate the tasks proposed in FluidLab. FluidEngine is a general-purpose physics simulator that supports modeling solid, liquid and gas, covering materials including elastic, plastic and rigid objects, Newtonian and non-Newtonian liquid, as well as smoke or air. FluidEngine is developed using Taichi \citep{hu2019taichi}, a domain-specific language embedded in Python, and supports massive parallelism on GPUs. In addition, it is implemented in a fully \textit{differentiable} manner, providing useful gradient information for downstream optimization tasks. Notably, closest to FluidEngine is Nvidia FleX \citep{macklin2014unified}, a physics engine that supports both rigid and deformable objects and is widely used in a variety of manipulation environments \citep{lin2020softgym, gan2020threedworld, schenck2018spnets}. However, FleX doesn't support simulating plastic materials and air, and is not differentiable. FluidEngine follows the standard OpenAI Gym API \citep{brockman2016openai} and also comes with a user-friendly Python interface for building custom environments. In addition, we provide a GPU-accelerated renderer developed with OpenGL, providing realistic image rendering in real-time and opening possibilities for sim-to-real transfer in the future. We discuss the details of FluidEngine in Section \ref{sec:fluidengine} and the tasks proposed in FluidLab in Section \ref{sec:fluidlab}. 

\todo{Bo: I guess this paragraph is mainly for optimization? I feel the current writting was a simple duplication of the abstract and no extra information was provided (also the language was vague in many places). We need to think about what to highlight here.}
We evaluate several state-of-the-art Reinforcement Learning algorithms and optimization methods in FluidLab, and show the \todo{blah blah}. In addition, since differentiable physics has proved useful in many rigid-body and soft-body robotic tasks \citep{xu2021end, lin2022diffskill, xu2022accelerated, li2022contact}, it is desirable to extend it to fluid manipulation tasks. However, supporting such a wide spectrum of materials present in FluidLab in a differentiable way is extremely challenging, and optimization using the gradients is also difficult due to the highly non-smooth optimization landscapes of the proposed tasks.  We propose various techniques that are generally applicable to the context of fluids, making our simulation fully differentiable and providing useful methods to utilize these gradients for downstream optimizations tasks, even with highly unconvex landscapes. \todo{Bo: duplicated sentence.} We demonstrate that our proposed techniques, combined with differentiable physics, could be effective in solving a set of challenging tasks, even in those with highly unstable fluids, such as air. 


In summary, the contributions of this work are as follows:
\todo{Bo: How about four contributions? FluidLab, simulation, optimization, and test cases. I organized the current abstract in this way.}
\begin{itemize}
  % \item We formally formulate the problem of \textit{fluid manipulation}, categorize a set of complex robotic manipulation problems involving fluids under this formulation, and systematically study them.
  \item We propose \textit{FluidLab}, a set of standardized manipulation tasks for systematically study the problem of \textit{complex fluid manipulation} with challenging task settings and complex goal configurations.
 
  \item We present \textit{FluidEngine}, the underlying physics engine of FluidLab that makes it possible to model various material types required in FluidLab's tasks. To the best of our knowledge, it is the first-of-its-kind physics engine that supports such a wide spectrum of materials and allows multi-way coupling \todo{bo: is this phrase correct?} between them, while being \textit{fully differentiable}.
  
   \item We benchmark existing RL algorithms and optimization approaches, and propose techniques that make differentiable physics useful in solving a set of challenging tasks. Our experiments highlight several challenges for existing methods. We hope FluidLab could inspire future research to develop better methods for solving complex fluid manipulation tasks.
\end{itemize}



==> 2_intro_xian.tex <==
\section{Introduction} 
Imagine you are fishing in a peaceful lake. Your hat falls into the water, and starts to float out of reach. In order to get it back, you use your hands to paddle the water gently, making a current that pulls the the hat back into reach. Under this scenario, the water functions as a transmitting medium to accomplish the manipulation task. In fact, from making latte art and washing dishes, to designing smoke ventilation systems and pouring ketchup to chips, many of our everyday tasks involve interacting with different types of fluids. However, performing these tasks are still beyond reach of today's robotic systems due to several major challenges. First, it requires a high dimensional state space to fully describe a system with fluids in an informative way \citep{lin2020softgym}. Second, such systems have highly unstructured and complex underlying dynamics \citep{schenck2018spnets}. Third, a wide spectrum of different fluid types with a great variation in their properties \todo{Bo: some citations?} are present in our life. For example, while ketchup and smoke both share the first two aforementioned challenges, they also behave in a drastically different way.

Past decades have witnessed rapid progresses in robotic control and manipulation. Robotic systems today are able to perform reasonably well in a wide range of manipulation tasks including object pushing \citep{yu2016more, li2018push, tung20203d}, grasping and pick-and-place \citep{kleeberger2020survey, zeng2020transporter, shridhar2022cliport}, dexterous and in-hand manipulation \citep{andrychowicz2020learning, chen2022system}, and even furniture assembly \citep{suarez2018can, lee2021ikea}. However, most of these tasks mainly consider rigid objects and focus on goal configurations represented as inter-object spatial relationships. In recent years, there has been a developing interest in manipulating deformable and articulated objects \citep{nair2017combining, schenck2018spnets, li2018learning, lin2020softgym, huang2021plasticinelab, lin2022diffskill, wu2021vat}, where intra-body configurations and appearances of these objects are taken into account during manipulation. Some work among them also cover manipulation tasks involving fluids \citep{ma2018fluid, lin2020softgym, antonova2022rethinking}, but mostly adopts relatively simple task settings, and usually considers tasks with a single-phase fluid, such as pouring water \citep{schenck2018spnets, lin2020softgym, sermanet2018time} or scooping objects from water \citep{Daniel2022toolflow, antonova2022rethinking}. In this work, we aim to take one step further and study the problem of \textit{complex fluid manipulation} with more challenging task settings and complex goal configurations.

To this end, we propose \textit{FluidLab}, a simulation environment with a comprehensive set of manipulation tasks involving various types of fluids. These tasks are motivated by scenarios encountered in our daily life, and consider both interactions within a multi-phase fluid body, as well as coupling between fluid and non-fluid bodies. Building such an environment poses a major challenge to the simulation capability: fluids encountered in our life consist of a wide spectrum of materials with different properties; in addition, simulating these tasks also requires modeling interactions with other non-fluid bodies. For example, coffee is \textit{non-viscous Newtonian} liquid, frothed milk behaves as \textit{viscous Newtonian} liquid, while ice-cream is a type of \textit{non-Newtonian} fluid; when stirring a cup of coffee, we use a \textit{rigid} stirrer to manipulate the coffee. However, there lacks a simulation engine in the research community that supports such a wide variety of materials and coupling between them. Therefore, we developed our own physics engine, named \textit{FluidEngine}, to support the tasks proposed in FluidLab. FluidEngine is a general-purpose physics simulator that supports modeling solid, liquid and gas, covering materials including elastic, plastic and rigid objects, Newtonian and non-Newtonian liquid, as well as smoke or air. FluidEngine is developed using Taichi \citep{hu2019taichi}, a domain-specific language embedded in Python, and supports massive parallelism on GPUs. In addition, it is implemented in a fully \textit{differentiable} manner, providing useful gradient information for downstream optimization tasks. Notably, closest to FluidEngine is Nvidia FleX \citep{macklin2014unified}, a physics engine that supports both rigid and deformable objects and is widely used in a variety of manipulation environments \citep{lin2020softgym, gan2020threedworld, schenck2018spnets}. However, FleX doesn't support simulating plastic materials and air, and is not differentiable either. FluidEngine follows the standard OpenAI Gym API \citep{brockman2016openai} and also comes with a user-friendly Python interface for building custom environments. In addition, we provide a GPU-accelerated renderer developed with OpenGL, providing realistic image rendering in real-time and opens possibility for sim-to-real transfer in the future. We discuss the details of FluidEngine in Section \ref{sec:fluidengine} and the tasks proposed in FluidLab in Section \ref{sec:fluidlab}. 

We evaluate several state-of-the-art Reinforcement Learning algorithms and optimization methods in FluidLab, and show the \todo{blah blah}. In addition, since differentiable physics has proved useful in many rigid-body and soft-body robotic tasks \citep{xu2021end, lin2022diffskill, xu2022accelerated, li2022contact}, it is desirable to extend it to fluid manipulation tasks. However, supporting such a wide spectrum of materials present in FluidLab in a differentiable way is extremely challenging, and optimization using the gradients is also difficult due to the highly non-smooth optimization landscapes of the proposed tasks.  We propose various techniques that are generally applicable to the context of fluids, making our simulation fully differentiable and providing useful methods to utilize these gradients for downstream optimizations tasks, even with highly unconvex landscapes. We demonstrate that our proposed techniques, combined with differentiable physics, could be effective in solving a set of challenging tasks, even in those with highly unstable fluids, such as air. 


In summary, the contributions of this work are as follows:

\begin{itemize}
  % \item We formally formulate the problem of \textit{fluid manipulation}, categorize a set of complex robotic manipulation problems involving fluids under this formulation, and systematically study them.
  \item We propose \textit{FluidLab}, a set of standardized manipulation tasks for systematically study the problem of \textit{complex fluid manipulation} with challenging task settings and complex goal configurations.
 
  \item We present \textit{FluidEngine}, the underlying physics engine of FluidLab that makes it possible to model various material types required in FluidLab's tasks. To the best of our knowledge, it is the first-of-its-kind physics engine that supports such a wide spectrum of materials and allows multi-way coupling \todo{bo: is this phrase correct?} between them, while being \textit{fully differentiable}.
  
   \item We benchmark existing RL algorithms and optimization approaches, and propose techniques that make differentiable physics useful in solving a set of challenging tasks. Our experiments highlight several challenges for existing methods. We hope FluidLab could inspire future research to develop better methods for solving complex fluid manipulation tasks.
\end{itemize}


\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth,height=6cm]{figures/fluidmanipulation.png}
\caption{Fluidmanipulation}
\label{fig:tasks}
\end{figure*}


==> 3_related_xian.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Robotic manipulation of rigid bodies, soft bodies and fluids}
Robotic manipulation has been extensively studies over the past decades, while most of previous works concern tasks settings with mainly rigid objects \citep{yu2016more, zeng2020transporter, shridhar2022cliport, suarez2018can, chen2022system}. In recent years, there has been a rising interest in manipulation problems concerning systems with deformable objects, which are generally more challenging than rigid-body manipulation problems due to the higher dimensional observation space and more complex dynamics. In these works, various types of deformable objects were studied, including elastic objects such as rope \citep{nair2017combining, yan2020self, lin2020softgym} and cloth \citep{liang2019differentiable, wu2019learning, lin2022learning}, as well as plastic objects like plasticine \citep{huang2021plasticinelab} and dough \citep{lin2022diffskill}. Some of them also studies manipulation problems involving fluids, but most of them only consider relatively simple problems settings such as robotic pouring \citep{lin2020softgym, narasimhan2022self} or scooping \citep{antonova2022rethinking}, and mostly deal with only water \citep{li2018learning, schenck2018spnets, ma2018fluid}. There exist some contemporary works that also study manipulation with fluids \citep{Daniel2022toolflow, antonova2022rethinking}, but are still restricted to tasks like scooping objects from water. In this work, we aim to study a comprehensive set of manipulation tasks involving different fluid types with various properties. It is also worth mentioning that aside from the robotics community, various previous work have also attempted to deal with fluid control problems in the computer graphics community \citep{hu2019difftaichi, mcnamara2004fluid, zhu2011sketch, yang2013unified}, but they mainly assume access to arbitrary control within the fluid body, e.g. control over velocity, force or mass field.\todo{Bo: maybe help a bit with this sentence?} Contrast to them, we study fluid manipulation from a realistic \textit{robotics} perspective, where fluids are manipulated with an embodied robotic agent equipped with some forms of physical end-effectors.

\paragraph{Simulation environments for robotic policy learning}
In recent years, simulation environments and standardized benchmarks have significantly facilitated research in robotics and policy learning. However, most of them \citep{brockman2016openai, kolve2017ai2, xiang2020sapien} use either PyBullet \citep{coumans2019} or MuJoCo \citep{todorov2012mujoco} as their underlying physics engines, which only supports rigid-body simulation. Recently, environments supporting soft-body manipulation, such as SAPIEN \citep{xiang2020sapien}, TDW \citep{gan2020threedworld} and SoftGym \citep{lin2020softgym} adopted Nvidia FleX \citep{macklin2014unified} engine to simulate deformable objects and fluids. However, FleX only supports limited types of materials, and its underlying Position-Based Dynamics (PBD) solver has been considered not physically accurate enough to reproduce faithful material behaviors \todo{bo: help with this sentence}. We provide a detailed comparison with these simulation engine and environments in Section \ref{sec:fluidengine}.

\paragraph{Differentiable physics simulation}
Machine Learning with differentiable physics has gained increasing attention recently. One line of research focuses on learning physics models with neural networks \cite{li2018learning, sanchez2020learning, pfaff2020learning}, which are intrinsically differentiable and could be used for downstream planning and optimization. Learning these models assumes ground-truth physic data provided by simulators, hasn't prove to be capable of simulating a wide range of materials, and could suffer from out-of-domain generalization accuracy \todo{katerina: some help here?}. Another approach is to implement physics simulations in a differentiable manner, usually with automatic differentiation tools \citep{hu2019difftaichi, de2018end, xu2022accelerated, huang2021plasticinelab}, and the gradient information provided by these simulations proves to be helpful in control and manipulation tasks concerning rigid and soft bodies \citep{xu2021end, lin2022diffskill, xu2022accelerated, li2022contact, huang2021plasticinelab}.  Our work aims to study manipulation problems with various forms of fluids and their coupling with other materials, and investigate the role of differentiable physics under this context. On a related note, Taichi \citep{hu2019taichi} and Nvidia Warp \citep{warp2022} are two recently developed domain-specific programming language for GPU-accelerated simulation. FluidLab is implemented using Taichi.

==> 7_discussion.tex <==
\section{Discussion on Potential Research Problems}

==> fluidenv_code.tex <==

\begin{lstlisting}[language=Python]
import os
import gym
import numpy as np
from gym.spaces import Box
from fluidlab.configs.macros import *
from fluidlab.engine.scenes import Scene
import fluidlab.utils.misc as misc_utils

class FluidEnv(gym.Env):
    '''
    Base env class.
    '''    
    def __init__(self, version, loss=True, loss_type='diff', seed=None):
        if seed is not None:
            self.seed(seed)

        self.horizon               = 500
        self.horizon_action        = 500
        self.target_file           = None
        self._n_obs_ptcls_per_body = 200
        self.loss                  = loss
        self.loss_type             = loss_type
        self.action_range          = np.array([-1.0, 1.0])

        # create a simulation
        self.scene = Scene()
        self.build_env()
        self.gym_misc()

    def seed(self, seed):
        super(FluidEnv, self).seed(seed)
        misc_utils.set_random_seed(seed)

    def build_env(self):
        self.setup_agent()
        self.setup_statics()
        self.setup_bodies()
        self.setup_gas_field()
        self.setup_boundary()
        self.setup_renderer()
        self.setup_loss()
            
        self.scene.build()
        self._init_state = self.scene.get_state()
        
        print(f'===>  {type(self).__name__} built successfully.')

    def setup_agent(self):
        agent_cfg = CfgNode(new_allowed=True)
        agent_cfg.merge_from_file(get_cfg_path('agent_scooping.yaml'))
        self.scene.setup_agent(agent_cfg)
        self.agent = self.scene.agent

    def setup_statics(self):
        # add static mesh-based objects in the scene
        self.scene.add_static(
            file='tank.obj',
            pos=(0.5, 0.4, 0.5),
            euler=(0.0, 0.0, 0.0),
            scale=(0.85, 0.92, 0.92),
            material=TANK,
            has_dynamics=False,
        )

    def setup_bodies(self):
        # add fluid/object bodies
        self.scene.add_body(
            type='cube',
            lower=(0.12, 0.25, 0.18),
            upper=(0.88, 0.45, 0.82),
            material=WATER,
        )
        self.scene.add_body(
            type='mesh',
            file='duck.obj',
            pos=(0.5, 0.6, 0.55),
            scale=(0.10, 0.10, 0.10),
            euler=(0, -90.0, 0.0),
            color=(1.0, 1.0, 0.3, 1.0),
            filling='grid',
            material=ELASTIC,
        )
        self.scene.add_body(
            type='cylinder',
            center=(0.2, 0.5, 0.55),
            height=0.08,
            radius=0.02,
            euler=(0.0, 0.0, -45.0),
            color=(1.0, 0.5, 0.5, 1.0),
            filling='natural',
            material=ELASTIC,
        )

    def setup_gas_field(self):
        self.scene.setup_gas_field(
            res          = 128,
            dt           = 0.03,
            solver_iters = 50,
            decay        = 0.99,
            q_dim        = 1,
        )
        
    def setup_boundary(self):
        self.scene.setup_boundary(
            type='cube',
            lower=(0.12, 0.25, 0.18),
            upper=(0.88, 0.95, 0.82),
        )

    def setup_renderer(self):
        self.scene.setup_renderer()

    def setup_loss(self):
        pass

    def gym_misc(self):
        obs = self.reset()
        self.observation_space = Box(DTYPE_NP(-np.inf), DTYPE_NP(np.inf), obs.shape, dtype=DTYPE_NP)
        if self.scene.agent is not None:
            self.action_space = Box(DTYPE_NP(self.action_range[0]), DTYPE_NP(self.action_range[1]), (self.scene.agent.action_dim,), dtype=DTYPE_NP)
        else:
            self.action_space = None

    def reset(self):
        self.scene.set_state(**self._init_state)
        return self._get_obs()

    def step(self, action):
        self.scene.step(action)

        obs    = self._get_obs()
        reward = self._get_reward()

        assert self.t <= self.horizon
        if self.t == self.horizon:
            done = True
        else:
            done = False

        info = dict()
        return obs, reward, done, info

    def render(self, mode='human'):
        assert mode in ['human', 'rgb_array']
        return self.scene.render(mode)

        
\end{lstlisting}
